Image-Space Refraction Correction for Underwater 3D Reconstruction: Warping Flat-Port Views into Pinhole Perspective

Consumer-grade cameras in flat-port housings are widely used for underwater exploration and mapping of coral reefs and seafloor habitats due to their low cost and accessibility. However, refraction at flat-port interfaces causes bowl-shaped deformation in reconstructed scenes and camera trajectories, compromising the metric accuracy required for mapping and navigation. To remove the dominant refractive distortion before reconstruction, we introduce a physics-based refraction correction in image space. Our method is downstream-agnostic: the refraction-corrected images can be directly used as input to existing reconstruction and SLAM algorithms. We characterize the refractive distortion through ray-tracing simulations and validate our correction on two real underwater datasets with differing scene structures. Compared with conventional and refractive Structure-from-Motion (SfM), our approach removes reconstruction deformation while registering more frames and maintaining low reprojection error. The correction further generalizes across diverse reconstruction and VSLAM backends, demonstrating its broad applicability to downstream vision pipelines.

==> tables/results_main_backup.tex <==
\newcommand{\tbox}[1]{{\setlength{\fboxsep}{1pt}\boxed{#1}}}

\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Reconstruction results}. Distortion parameters are held fixed (\emph{fix}) or refined (\emph{ref}). Planarity is measured against the scene (Malaysia) or trajectory (Lizard Island). $\kappa = 0$ indicates a flat reconstruction; negative values correspond to a bowl and positive values to a dome.}
\label{tab:main_results}

\centering
\textbf{Lizard Island}\\[2pt]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllccccc}
\toprule
Sequence & Method & Dist. & Reg.$\uparrow$ & Pts$^{\times 10^5}\uparrow$ & Track$\uparrow$ & Reproj.$\downarrow$ & $\kappa \approx 0$ \\
\midrule
\multirow{4}{*}{feb\_gp1}
& COLMAP & fix &  0.86 & 4.92 & 4.60 & 1.21 & $-0.290$ \\
& COLMAP & ref & 0.88 & 4.22 & 6.78 & 0.35 & $+0.366$ \\
& Refractive COLMAP & fix & 0.88 & 4.22 & 6.77 & 0.36 & $-0.453$ \\
& Ours + COLMAP & fix & \underline{0.96} & \underline{5.85} & \underline{7.75} & \underline{0.34} &  $\tbox{\mathbf{+0.017}}$ \\
\midrule
\multirow{4}{*}{mar\_gp1}
& COLMAP & fix & 0.99 & \underline{9.33} & 4.83 & 1.33 & $+1.084$  \\
& COLMAP & ref & 0.99 & 6.72 & 8.35 & 0.48 & $+0.304$\\
& Refractive COLMAP & fix & 0.99 & 6.68 & 8.34 & 0.48 & $+0.055$ \\
& Ours + COLMAP & fix & \underline{1.00} & 8.15 & \underline{9.41} & \underline{0.45} & $\tbox{\mathbf{+0.014}}$ \\
\midrule
\multirow{4}{*}{mar\_gp2}
& COLMAP & fix & 0.87 & \underline{7.45} & 4.87 & 1.30 & $+0.090$ \\
& COLMAP & ref & 0.90 & 5.99 & 7.90 & 0.48 & $-0.306$ \\
& Refractive COLMAP & fix & 0.90 & 5.98 & 7.88 & 0.48 & $-0.057$ \\
& Ours + COLMAP & fix & \underline{1.00} & 6.99 & \underline{9.25} & \underline{0.47} & $\tbox{\mathbf{+0.017}}$ \\
\midrule
\multirow{4}{*}{sep\_gp1}
& COLMAP & fix & 0.76 & \underline{7.33} & 4.96& 1.38 & $-0.818$ \\
& COLMAP & ref & 0.79 & 5.10 & 9.19 & 0.57 & $-0.082$ \\
& Refractive COLMAP & fix & 0.79 & 5.10 & 9.16 & 0.57 & $+0.045$ \\
& Ours + COLMAP & fix & \underline{0.97} & 6.93 & \underline{9.94} & \underline{0.52} & $\tbox{\mathbf{-0.024}}$ \\
\midrule
\multirow{4}{*}{sep\_gp2}
& COLMAP & fix & 0.39 & (5.10) & (4.44) & (1.36) & ($+2.068$) \\
& COLMAP & ref & 0.39 & (3.41) & (8.54) & (0.56) & ($-0.029$) \\
& Refractive COLMAP & fix & 0.39 & (3.41) & (8.52) & (0.56) & ($-0.068$) \\
& Ours + COLMAP & fix & \underline{0.83} & \underline{6.79} & \underline{8.84} & \underline{0.49} & $\tbox{\mathbf{+0.053}}$ \\
\bottomrule
\end{tabular}%
}

\vspace{8pt}

\centering
\textbf{Malaysia}\\[2pt]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lllccccc}
\toprule
Sequence & Method & Dist. & Reg.$\uparrow$ & Pts$^{\times 10^5}\uparrow$ & Track$\uparrow$ & Reproj.$\downarrow$ & $\kappa \approx 0$ \\
\midrule
\multirow{4}{*}{p1\_s01}
& COLMAP & fix & 0.95 & 24.68 & 5.16 & 0.75 & $+0.493$ \\
& COLMAP & ref & 0.95 & 23.32 & 5.70 & 0.37 & $+0.188$ \\
& Refractive COLMAP & fix & 0.95 & 22.42 & 5.43 & 0.68 & $+0.011$ \\
& Ours + COLMAP & fix & \underline{0.99} & \underline{27.37} &  \underline{6.01} & \underline{0.37} & $\tbox{\mathbf{-0.068}}$ \\
\midrule
\multirow{4}{*}{p1\_s02}
& COLMAP & fix & 1.00 &  \underline{14.58} & 6.32 & 0.60 & $+1.202$ \\
& COLMAP & ref & 1.00 & 12.70 & 7.38 & \underline{0.29} & $+0.089$ \\
& Refractive COLMAP & fix & 1.00 & 12.82 & 7.19 & 0.57 & $+0.694$ \\
& Ours + COLMAP & fix & 1.00 & 13.14 & \underline{8.57} & 0.32 & $\tbox{\mathbf{+0.000}}$ \\
\midrule
\multirow{4}{*}{p1\_s03}
& COLMAP & fix & 1.00 &  \underline{14.17} & 7.15 & 0.70 & $-1.378$ \\
& COLMAP & ref & 1.00 & 11.10 & 9.43 & \underline{0.36} & $+0.073$ \\
& Refractive COLMAP & fix & 1.00 & 11.41 & 8.94 & 0.68 & $+0.105$ \\
& Ours + COLMAP & fix & 1.00 & 10.61 & \underline{12.01} & 0.40 & $\tbox{\mathbf{+0.031}}$ \\
\midrule
\multirow{4}{*}{p3\_s02}
& COLMAP & fix & 1.00 & 13.89 & 4.50 & 0.65 & $-0.152$ \\
& COLMAP & ref & 1.00 & 12.97 & 5.03 & \underline{0.41} & $+0.064$ \\
& Refractive COLMAP & fix & 1.00 & 13.12 & 4.86 & 0.61 & $+0.025$ \\
& Ours + COLMAP & fix & 1.00 &  \underline{15.56} & \underline{5.40} & 0.42 & $\tbox{\mathbf{-0.004}}$ \\
\midrule
\multirow{4}{*}{p3\_s03}
& COLMAP & fix & 1.00 &  \underline{8.28} & 6.44 & 0.67 & $-2.047$ \\
& COLMAP & ref & 1.00 & 7.30 & 7.45 & \underline{0.35} & $-0.097$ \\
& Refractive COLMAP & fix & 1.00 & 7.32 & 7.34 & 0.62 & $+0.253$ \\
& Ours + COLMAP & fix & 1.00 & 7.76 & \underline{8.73} & 0.38 &$\tbox{\mathbf{+0.078}}$ \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/table_ablation1.tex <==
\begin{table}[t]
\centering
\caption{Depth ablation to find the optimal reference depth $Z_0$ for our method, on one Malaysia sequence (p1\_s02) and one Lizard Island sequence (feb\_gp1). We report track length, reprojection error, and curve/bending as $Z_0$ is varied.}
\label{tab:depth_ablation}

\centering
\textbf{Malaysia (p1\_s02)}\\[2pt]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
Metric & \multicolumn{9}{c}{$Z_0$ (m)} \\
\cmidrule(lr){2-10}
 & 0.25 & 0.5 & 1.0 & 1.5 & 1.75 & 2.0 & 5.0 & 10.0 & 50.0 \\
\midrule
Track   & 8.51 & 8.55 & 8.56 & 8.57 & 8.57 & 8.58 & 8.58 & 8.59 & -- \\
Reproj. & 0.371 & 0.338 & 0.325 & 0.321 & 0.320 & 0.319 & 0.316 & 0.315 & -- \\
Curve   & -0.386 & -0.170 & -0.052 & -0.012 & \textbf{0.000} & 0.008 & 0.046 & 0.059 & -- \\
\bottomrule
\end{tabular}%
}

\vspace{8pt}

\centering
\textbf{Lizard Island (feb\_gp1)}\\[2pt]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
Metric & \multicolumn{10}{c}{$Z_0$ (m)} \\
\cmidrule(lr){2-11}
 & 0.25 & 0.5 & 1.0 & 1.5 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 50.0 \\
\midrule
Track   & 5.75 & 5.76 & 5.77 & 5.78 & 5.77 & 5.77 & 5.77 & 5.76 & 5.77 & 5.77 \\
Reproj. & 0.336 & 0.296 & 0.293 & 0.295 & 0.296 & 0.297 & 0.298 & 0.299 & 0.301 & 0.303 \\
Curve   & -0.572 & -0.749 & -0.189 & -0.090 & -0.045 & \textbf{-0.001} & 0.023 & 0.037 & 0.064 & 0.087 \\
\bottomrule
\end{tabular}%
}
\end{table}

